Fast Second-order Cone Programming for Safe Mission Planning

This paper considers the problem of safe mission planning of dynamic systems operating under uncertain environments. Much of the prior work on achieving robust and safe control requires solving second-order cone programs (SOCP). Unfortunately, existing general purpose SOCP methods are often infeasible for real-time robotic tasks due to high memory and computational requirements imposed by existing general optimization methods. The key contribution of this paper is a fast and memory-efficient algorithm for SOCP that would enable robust and safe mission planning on-board robots in real-time. Our algorithm does not have any external dependency, can efficiently utilize warm start provided in safe planning settings, and in fact leads to significant speed up over standard optimization packages (like SDPT3) for even standard SOCP problems. For example, for a standard quadrotor problem, our method leads to speedup of 1000x over SDPT3 without any deterioration in the solution quality. Our method is based on two insights: a) SOCPs can be interpreted as optimizing a function over a polytope with infinite sides, b) a linear function can be efficiently optimized over this polytope. We combine the above observations with a novel utilization of Wolfe's algorithm to obtain an efficient optimization method that can be easily implemented on small embedded devices. In addition to the above mentioned algorithm, we also design a two-level sensing method based on Gaussian Process for complex obstacles with non-linear boundaries such as a cylinder.

==> rofu-defs.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\let\proof\relax
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{stmaryrd}
\RequirePackage{environ}
\RequirePackage{graphics}

\makeatletter
\@ifpackageloaded{dsfont}{}{\newcommand{\mathds}[1]{\mathbb{#1}}}
\@ifpackageloaded{mathrsfs}{}{\newcommand{\mathscr}[1]{\mathcal{#1}}}
\makeatother

%%%%%%%% Environment %%%%%%%%%%%%%

% \begin{resize}[height]{width} \end{resize}
 \NewEnviron{resize}[2][!]{\resizebox{#2}{#1}{\BODY}} 
% \begin{rescale}[height_ratio]{width_ratio} \end{rescale}
 \NewEnviron{rescale}[2][]{\scalebox{#2}[#1]{\BODY}}

\makeatletter
\newcommand{\newreptheorem}[2]{
  \newtheorem*{rep@#1}{\rep@title} 
  \newenvironment{rep#1}[1]{\def\rep@title{#2 \ref*{##1}}\begin{rep@#1}}{\end{rep@#1}}
}
\makeatother
\newreptheorem{theorem}{Theorem}
\newreptheorem{claim}{Claim}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

% matrix with original font/boldsymbol/mathcal and tilde/bar/hat
\newcommand{\ab}{{\bm{a}}}
\newcommand{\bb}{{\bm{b}}}
\newcommand{\cbb}{{\bm{c}}}
\newcommand{\db}{{\bm{d}}}
\newcommand{\eb}{{\bm{e}}}
\newcommand{\fb}{{\bm{f}}}
\newcommand{\gb}{{\bm{g}}}
\newcommand{\hb}{{\bm{h}}}
\newcommand{\ib}{{\bm{i}}}
\newcommand{\jb}{{\bm{j}}}
\newcommand{\kb}{{\bm{k}}}
\newcommand{\lb}{{\bm{l}}}
\newcommand{\mb}{{\bm{m}}}
\newcommand{\nbb}{{\bm{n}}}
\newcommand{\ob}{{\bm{o}}}
\newcommand{\pb}{{\bm{p}}}
\newcommand{\qb}{{\bm{q}}}
\newcommand{\rb}{{\bm{r}}}
\newcommand{\sbb}{{\bm{s}}}
\newcommand{\tb}{{\bm{t}}}
\newcommand{\ub}{{\bm{u}}}
\newcommand{\vb}{{\bm{v}}}
\newcommand{\wb}{{\bm{w}}}
\newcommand{\xb}{{\bm{x}}}
\newcommand{\yb}{{\bm{y}}}
\newcommand{\zb}{{\bm{z}}}

\newcommand{\ba}{\ab}
\newcommand{\bc}{\cbb}
\newcommand{\bd}{\db}
\newcommand{\be}{\eb}
\newcommand{\bbf}{\fb}
\newcommand{\bff}{\fb}
\newcommand{\bg}{\gb}
\newcommand{\bh}{\hb}
\newcommand{\bi}{\ib}
\newcommand{\bj}{\jb}
\newcommand{\bk}{\kb}
\newcommand{\bl}{\lb}
\newcommand{\bbm}{\mb}
\newcommand{\bmm}{\mb}
\newcommand{\bn}{\nbb}
\newcommand{\bo}{\ob}
\newcommand{\bp}{\pb}
\newcommand{\bq}{\qb}
\newcommand{\br}{\rb}
\newcommand{\bs}{\sbb}
\newcommand{\bt}{\tb}
\newcommand{\bu}{\ub}
\newcommand{\bv}{\vb}
\newcommand{\bw}{\wb}
\newcommand{\bx}{\xb}
\newcommand{\by}{\yb}
\newcommand{\bz}{\zb}

% version with tilde
\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\at}{\tilde{a}}
\newcommand{\bti}{\tilde{b}}
%\newcommand{\btt}{\tilde{b}}
\newcommand{\ct}{\tilde{c}}
\newcommand{\dt}{\tilde{d}}
\newcommand{\et}{\tilde{e}}
\newcommand{\ft}{\tilde{f}}
\newcommand{\gt}{\tilde{g}}
\newcommand{\hti}{\tilde{h}}
\newcommand{\htt}{\tilde{h}}
\newcommand{\iti}{\tilde{i}}
\newcommand{\itt}{\tilde{i}}
\newcommand{\jt}{\tilde{j}}
\newcommand{\kt}{\tilde{k}}
\newcommand{\lt}{\tilde{l}}
\newcommand{\mt}{\tilde{m}}
\newcommand{\nt}{\tilde{n}}
\newcommand{\ot}{\tilde{o}}
\newcommand{\pti}{\tilde{p}}
\newcommand{\ptt}{\tilde{p}}
\newcommand{\qt}{\tilde{q}}
\newcommand{\rt}{\tilde{r}}
\newcommand{\st}{\tilde{s}}
\newcommand{\tti}{\tilde{t}}
\newcommand{\ttt}{\tilde{t}}
\newcommand{\ut}{\tilde{u}}
\newcommand{\vti}{\tilde{v}}
\newcommand{\vtt}{\tilde{v}}
\newcommand{\wt}{\tilde{w}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\zt}{\tilde{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\batil}{\tilde{\ab}}
\newcommand{\bctil}{\tilde{\cbb}}
\newcommand{\bdtil}{\tilde{\db}}
\newcommand{\betil}{\tilde{\eb}}
\newcommand{\bftil}{\tilde{\fb}}
\newcommand{\bgtil}{\tilde{\gb}}
\newcommand{\bhtil}{\tilde{\hb}}
\newcommand{\bitil}{\tilde{\ib}}
\newcommand{\bjtil}{\tilde{\jb}}
\newcommand{\bktil}{\tilde{\kb}}
\newcommand{\bltil}{\tilde{\lb}}
\newcommand{\bmtil}{\tilde{\mb}}
\newcommand{\bntil}{\tilde{\nbb}}
\newcommand{\botil}{\tilde{\ob}}
\newcommand{\bptil}{\tilde{\pb}}
\newcommand{\bqtil}{\tilde{\qb}}
\newcommand{\brtil}{\tilde{\rb}}
\newcommand{\bstil}{\tilde{\sbb}}
\newcommand{\bttil}{\tilde{\tb}}
\newcommand{\butil}{\tilde{\ub}}
\newcommand{\bvtil}{\tilde{\vb}}
\newcommand{\bwtil}{\tilde{\wb}}
\newcommand{\bxtil}{\tilde{\xb}}
\newcommand{\bytil}{\tilde{\yb}}
\newcommand{\bztil}{\tilde{\zb}}

\newcommand{\bat}{\tilde{\ab}}
\newcommand{\bbt}{\tilde{\bb}}
\newcommand{\bct}{\tilde{\cbb}}
\newcommand{\bdt}{\tilde{\db}}
\newcommand{\bet}{\tilde{\eb}}
\newcommand{\bft}{\tilde{\fb}}
\newcommand{\bgt}{\tilde{\gb}}
\newcommand{\bht}{\tilde{\hb}}
\newcommand{\bit}{\tilde{\ib}}
\newcommand{\bjt}{\tilde{\jb}}
\newcommand{\bkt}{\tilde{\kb}}
\newcommand{\blt}{\tilde{\lb}}
\newcommand{\bmt}{\tilde{\mb}}
\newcommand{\bnt}{\tilde{\nbb}}
\newcommand{\boti}{\tilde{\ob}}
\newcommand{\boot}{\tilde{\ob}}
\newcommand{\bpt}{\tilde{\pb}}
\newcommand{\bqt}{\tilde{\qb}}
\newcommand{\brt}{\tilde{\rb}}
\newcommand{\bst}{\tilde{\sbb}}
\newcommand{\btti}{\tilde{\tb}}
\newcommand{\btt}{\tilde{\tb}}
\newcommand{\but}{\tilde{\ub}}
\newcommand{\bvt}{\tilde{\vb}}
\newcommand{\bwt}{\tilde{\wb}}
\newcommand{\bxt}{\tilde{\xb}}
\newcommand{\byt}{\tilde{\yb}}
\newcommand{\bzt}{\tilde{\zb}}

% version with hat
\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\bahat}{\hat{\ab}}
\newcommand{\bchat}{\hat{\bc}}
\newcommand{\bdhat}{\hat{\db}}
\newcommand{\behat}{\hat{\eb}}
\newcommand{\bfhat}{\hat{\fb}}
\newcommand{\bghat}{\hat{\gb}}
\newcommand{\bhhat}{\hat{\hb}}
\newcommand{\bihat}{\hat{\ib}}
\newcommand{\bjhat}{\hat{\jb}}
\newcommand{\bkhat}{\hat{\kb}}
\newcommand{\blhat}{\hat{\lb}}
\newcommand{\bmhat}{\hat{\mb}}
\newcommand{\bnhat}{\hat{\nbb}}
\newcommand{\bohat}{\hat{\ob}}
\newcommand{\bphat}{\hat{\pb}}
\newcommand{\bqhat}{\hat{\qb}}
\newcommand{\brhat}{\hat{\rb}}
\newcommand{\bshat}{\hat{\sbb}}
\newcommand{\bthat}{\hat{\tb}}
\newcommand{\buhat}{\hat{\ub}}
\newcommand{\bvhat}{\hat{\vb}}
\newcommand{\bwhat}{\hat{\wb}}
\newcommand{\bxhat}{\hat{\xb}}
\newcommand{\byhat}{\hat{\yb}}
\newcommand{\bzhat}{\hat{\zb}}

% version with bar
\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obr}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\babar}{\bar{\ab}}
\newcommand{\bcbar}{\bar{\bc}}
\newcommand{\bdbar}{\bar{\db}}
\newcommand{\bebar}{\bar{\eb}}
\newcommand{\bfbar}{\bar{\fb}}
\newcommand{\bgbar}{\bar{\gb}}
\newcommand{\bhbar}{\bar{\hb}}
\newcommand{\bibar}{\bar{\ib}}
\newcommand{\bjbar}{\bar{\jb}}
\newcommand{\bkbar}{\bar{\kb}}
\newcommand{\blbar}{\bar{\lb}}
\newcommand{\bmbar}{\bar{\mb}}
\newcommand{\bnbar}{\bar{\nbb}}
\newcommand{\bobar}{\bar{\ob}}
\newcommand{\bpbar}{\bar{\pb}}
\newcommand{\bqbar}{\bar{\qb}}
\newcommand{\brbar}{\bar{\rb}}
\newcommand{\bsbar}{\bar{\sbb}}
\newcommand{\btbar}{\bar{\tb}}
\newcommand{\bubar}{\bar{\ub}}
\newcommand{\bvbar}{\bar{\vb}}
\newcommand{\bwbar}{\bar{\wb}}
\newcommand{\bxbar}{\bar{\xb}}
\newcommand{\bybar}{\bar{\yb}}
\newcommand{\bzbar}{\bar{\zb}}

% matrix with original font/boldsymbol/mathcal and tilde/bar/hat
\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\At}{\tilde{A}}
\newcommand{\Bt}{\tilde{B}}
\newcommand{\Ct}{\tilde{C}}
\newcommand{\Dt}{\tilde{D}}
\newcommand{\Et}{\tilde{E}}
\newcommand{\Ft}{\tilde{F}}
\newcommand{\Gt}{\tilde{G}}
\newcommand{\Ht}{\tilde{H}}
\newcommand{\It}{\tilde{I}}
\newcommand{\Jt}{\tilde{J}}
\newcommand{\Kt}{\tilde{K}}
\newcommand{\Lt}{\tilde{L}}
\newcommand{\Mt}{\tilde{M}}
\newcommand{\Nt}{\tilde{N}}
\newcommand{\Ot}{\tilde{O}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Qt}{\tilde{Q}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\St}{\tilde{S}}
\newcommand{\Tt}{\tilde{T}}
\newcommand{\Ut}{\tilde{U}}
\newcommand{\Vt}{\tilde{V}}
\newcommand{\Wt}{\tilde{W}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Zt}{\tilde{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Ab}{\bm{{A}}}
\newcommand{\Bb}{\bm{{B}}}
\newcommand{\Cb}{\bm{{C}}}
\newcommand{\Db}{\bm{{D}}}
\newcommand{\Eb}{\bm{{E}}}
\newcommand{\Fb}{\bm{{F}}}
\newcommand{\Gb}{\bm{{G}}}
\newcommand{\Hb}{\bm{{H}}}
\newcommand{\Ib}{\bm{{I}}}
\newcommand{\Jb}{\bm{{J}}}
\newcommand{\Kb}{\bm{{K}}}
\newcommand{\Lb}{\bm{{L}}}
\newcommand{\Mb}{\bm{{M}}}
\newcommand{\Nb}{\bm{{N}}}
\newcommand{\Ob}{\bm{{O}}}
\newcommand{\Pb}{\bm{{P}}}
\newcommand{\Qb}{\bm{{Q}}}
\newcommand{\Rb}{\bm{{R}}}
\newcommand{\Sbb}{\bm{{S}}}
\newcommand{\Tb}{\bm{{T}}}
\newcommand{\Ub}{\bm{{U}}}
\newcommand{\Vb}{\bm{{V}}}
\newcommand{\Wb}{\bm{{W}}}
\newcommand{\Xb}{\bm{{X}}}
\newcommand{\Yb}{\bm{{Y}}}
\newcommand{\Zb}{\bm{{Z}}}

\newcommand{\bA}{\bm{{A}}}
\newcommand{\bB}{\bm{{B}}}
\newcommand{\bC}{\bm{{C}}}
\newcommand{\bD}{\bm{{D}}}
\newcommand{\bE}{\bm{{E}}}
\newcommand{\bF}{\bm{{F}}}
\newcommand{\bG}{\bm{{G}}}
\newcommand{\bH}{\bm{{H}}}
\newcommand{\bI}{\bm{{I}}}
\newcommand{\bJ}{\bm{{J}}}
\newcommand{\bK}{\bm{{K}}}
\newcommand{\bL}{\bm{{L}}}
\newcommand{\bM}{\bm{{M}}}
\newcommand{\bN}{\bm{{N}}}
\newcommand{\bO}{\bm{{O}}}
\newcommand{\bP}{\bm{{P}}}
\newcommand{\bQ}{\bm{{Q}}}
\newcommand{\bR}{\bm{{R}}}
\newcommand{\bS}{\bm{{S}}}
\newcommand{\bT}{\bm{{T}}}
\newcommand{\bU}{\bm{{U}}}
\newcommand{\bV}{\bm{{V}}}
\newcommand{\bW}{\bm{{W}}}
\newcommand{\bX}{\bm{{X}}}
\newcommand{\bY}{\bm{{Y}}}
\newcommand{\bZ}{\bm{{Z}}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\bAt}{\tilde{\Ab}}
\newcommand{\bBt}{\tilde{\Bb}}
\newcommand{\bCt}{\tilde{\Cb}}
\newcommand{\bDt}{\tilde{\Db}}
\newcommand{\bEt}{\tilde{\Eb}}
\newcommand{\bFt}{\tilde{\Fb}}
\newcommand{\bGt}{\tilde{\Gb}}
\newcommand{\bHt}{\tilde{\Hb}}
\newcommand{\bIt}{\tilde{\Ib}}
\newcommand{\bJt}{\tilde{\Jb}}
\newcommand{\bKt}{\tilde{\Kb}}
\newcommand{\bLt}{\tilde{\Lb}}
\newcommand{\bMt}{\tilde{\Mb}}
\newcommand{\bNt}{\tilde{\Nb}}
\newcommand{\bOt}{\tilde{\Ob}}
\newcommand{\bPt}{\tilde{\Pb}}
\newcommand{\bQt}{\tilde{\Qb}}
\newcommand{\bRt}{\tilde{\Rb}}
\newcommand{\bSt}{\tilde{\Sbb}}
\newcommand{\bTt}{\tilde{\Tb}}
\newcommand{\bUt}{\tilde{\Ub}}
\newcommand{\bVt}{\tilde{\Vb}}
\newcommand{\bWt}{\tilde{\Wb}}
\newcommand{\bXt}{\tilde{\Xb}}
\newcommand{\bYt}{\tilde{\Yb}}
\newcommand{\bZt}{\tilde{\Zb}}

\newcommand{\bAtil}{\tilde{\Ab}}
\newcommand{\bBtil}{\tilde{\Bb}}
\newcommand{\bCtil}{\tilde{\Cb}}
\newcommand{\bDtil}{\tilde{\Db}}
\newcommand{\bEtil}{\tilde{\Eb}}
\newcommand{\bFtil}{\tilde{\Fb}}
\newcommand{\bGtil}{\tilde{\Gb}}
\newcommand{\bHtil}{\tilde{\Hb}}
\newcommand{\bItil}{\tilde{\Ib}}
\newcommand{\bJtil}{\tilde{\Jb}}
\newcommand{\bKtil}{\tilde{\Kb}}
\newcommand{\bLtil}{\tilde{\Lb}}
\newcommand{\bMtil}{\tilde{\Mb}}
\newcommand{\bNtil}{\tilde{\Nb}}
\newcommand{\bOtil}{\tilde{\Ob}}
\newcommand{\bPtil}{\tilde{\Pb}}
\newcommand{\bQtil}{\tilde{\Qb}}
\newcommand{\bRtil}{\tilde{\Rb}}
\newcommand{\bStil}{\tilde{\Sbb}}
\newcommand{\bTtil}{\tilde{\Tb}}
\newcommand{\bUtil}{\tilde{\Ub}}
\newcommand{\bVtil}{\tilde{\Vb}}
\newcommand{\bWtil}{\tilde{\Wb}}
\newcommand{\bXtil}{\tilde{\Xb}}
\newcommand{\bYtil}{\tilde{\Yb}}
\newcommand{\bZtil}{\tilde{\Zb}}

\newcommand{\bAtilde}{\widetilde{\Ab}}
\newcommand{\bBtilde}{\widetilde{\Bb}}
\newcommand{\bCtilde}{\widetilde{\Cb}}
\newcommand{\bDtilde}{\widetilde{\Db}}
\newcommand{\bEtilde}{\widetilde{\Eb}}
\newcommand{\bFtilde}{\widetilde{\Fb}}
\newcommand{\bGtilde}{\widetilde{\Gb}}
\newcommand{\bHtilde}{\widetilde{\Hb}}
\newcommand{\bItilde}{\widetilde{\Ib}}
\newcommand{\bJtilde}{\widetilde{\Jb}}
\newcommand{\bKtilde}{\widetilde{\Kb}}
\newcommand{\bLtilde}{\widetilde{\Lb}}
\newcommand{\bMtilde}{\widetilde{\Mb}}
\newcommand{\bNtilde}{\widetilde{\Nb}}
\newcommand{\bOtilde}{\widetilde{\Ob}}
\newcommand{\bPtilde}{\widetilde{\Pb}}
\newcommand{\bQtilde}{\widetilde{\Qb}}
\newcommand{\bRtilde}{\widetilde{\Rb}}
\newcommand{\bStilde}{\widetilde{\Sbb}}
\newcommand{\bTtilde}{\widetilde{\Tb}}
\newcommand{\bUtilde}{\widetilde{\Ub}}
\newcommand{\bVtilde}{\widetilde{\Vb}}
\newcommand{\bWtilde}{\widetilde{\Wb}}
\newcommand{\bXtilde}{\widetilde{\Xb}}
\newcommand{\bYtilde}{\widetilde{\Yb}}
\newcommand{\bZtilde}{\widetilde{\Zb}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sbb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\bAbar}{\bar{\Ab}}
\newcommand{\bBbar}{\bar{\Bb}}
\newcommand{\bCbar}{\bar{\Cb}}
\newcommand{\bDbar}{\bar{\Db}}
\newcommand{\bEbar}{\bar{\Eb}}
\newcommand{\bFbar}{\bar{\Fb}}
\newcommand{\bGbar}{\bar{\Gb}}
\newcommand{\bHbar}{\bar{\Hb}}
\newcommand{\bIbar}{\bar{\Ib}}
\newcommand{\bJbar}{\bar{\Jb}}
\newcommand{\bKbar}{\bar{\Kb}}
\newcommand{\bLbar}{\bar{\Lb}}
\newcommand{\bMbar}{\bar{\Mb}}
\newcommand{\bNbar}{\bar{\Nb}}
\newcommand{\bObar}{\bar{\Ob}}
\newcommand{\bPbar}{\bar{\Pb}}
\newcommand{\bQbar}{\bar{\Qb}}
\newcommand{\bRbar}{\bar{\Rb}}
\newcommand{\bSbar}{\bar{\Sbb}}
\newcommand{\bTbar}{\bar{\Tb}}
\newcommand{\bUbar}{\bar{\Ub}}
\newcommand{\bVbar}{\bar{\Vb}}
\newcommand{\bWbar}{\bar{\Wb}}
\newcommand{\bXbar}{\bar{\Xb}}
\newcommand{\bYbar}{\bar{\Yb}}
\newcommand{\bZbar}{\bar{\Zb}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sbb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\bAhat}{\hat{\Ab}}
\newcommand{\bBhat}{\hat{\Bb}}
\newcommand{\bChat}{\hat{\Cb}}
\newcommand{\bDhat}{\hat{\Db}}
\newcommand{\bEhat}{\hat{\Eb}}
\newcommand{\bFhat}{\hat{\Fb}}
\newcommand{\bGhat}{\hat{\Gb}}
\newcommand{\bHhat}{\hat{\Hb}}
\newcommand{\bIhat}{\hat{\Ib}}
\newcommand{\bJhat}{\hat{\Jb}}
\newcommand{\bKhat}{\hat{\Kb}}
\newcommand{\bLhat}{\hat{\Lb}}
\newcommand{\bMhat}{\hat{\Mb}}
\newcommand{\bNhat}{\hat{\Nb}}
\newcommand{\bOhat}{\hat{\Ob}}
\newcommand{\bPhat}{\hat{\Pb}}
\newcommand{\bQhat}{\hat{\Qb}}
\newcommand{\bRhat}{\hat{\Rb}}
\newcommand{\bShat}{\hat{\Sbb}}
\newcommand{\bThat}{\hat{\Tb}}
\newcommand{\bUhat}{\hat{\Ub}}
\newcommand{\bVhat}{\hat{\Vb}}
\newcommand{\bWhat}{\hat{\Wb}}
\newcommand{\bXhat}{\hat{\Xb}}
\newcommand{\bYhat}{\hat{\Yb}}
\newcommand{\bZhat}{\hat{\Zb}}

% mathcal version 
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\Acaltil}{\tilde{\cA}}
\newcommand{\Bcaltil}{\tilde{\cB}}
\newcommand{\Ccaltil}{\tilde{\cC}}
\newcommand{\Dcaltil}{\tilde{\cD}}
\newcommand{\Ecaltil}{\tilde{\cE}}
\newcommand{\Fcaltil}{\tilde{\cF}}
\newcommand{\Gcaltil}{\tilde{\cG}}
\newcommand{\Hcaltil}{\tilde{\cH}}
\newcommand{\Icaltil}{\tilde{\cI}}
\newcommand{\Jcaltil}{\tilde{\cJ}}
\newcommand{\Kcaltil}{\tilde{\cK}}
\newcommand{\Lcaltil}{\tilde{\cL}}
\newcommand{\Mcaltil}{\tilde{\cM}}
\newcommand{\Ncaltil}{\tilde{\cN}}
\newcommand{\Ocaltil}{\tilde{\cO}}
\newcommand{\Pcaltil}{\tilde{\cP}}
\newcommand{\Qcaltil}{\tilde{\cQ}}
\newcommand{\Rcaltil}{\tilde{\cR}}
\newcommand{\Scaltil}{\tilde{\cS}}
\newcommand{\Tcaltil}{\tilde{\cT}}
\newcommand{\Ucaltil}{\tilde{\cU}}
\newcommand{\Vcaltil}{\tilde{\cV}}
\newcommand{\Wcaltil}{\tilde{\cW}}
\newcommand{\Xcaltil}{\tilde{\cX}}
\newcommand{\Ycaltil}{\tilde{\cY}}
\newcommand{\Zcaltil}{\tilde{\cZ}}

\newcommand{\cAtil}{\tilde{\cA}}
\newcommand{\cBtil}{\tilde{\cB}}
\newcommand{\cCtil}{\tilde{\cC}}
\newcommand{\cDtil}{\tilde{\cD}}
\newcommand{\cEtil}{\tilde{\cE}}
\newcommand{\cFtil}{\tilde{\cF}}
\newcommand{\cGtil}{\tilde{\cG}}
\newcommand{\cHtil}{\tilde{\cH}}
\newcommand{\cItil}{\tilde{\cI}}
\newcommand{\cJtil}{\tilde{\cJ}}
\newcommand{\cKtil}{\tilde{\cK}}
\newcommand{\cLtil}{\tilde{\cL}}
\newcommand{\cMtil}{\tilde{\cM}}
\newcommand{\cNtil}{\tilde{\cN}}
\newcommand{\cOtil}{\tilde{\cO}}
\newcommand{\cPtil}{\tilde{\cP}}
\newcommand{\cQtil}{\tilde{\cQ}}
\newcommand{\cRtil}{\tilde{\cR}}
\newcommand{\cStil}{\tilde{\cS}}
\newcommand{\cTtil}{\tilde{\cT}}
\newcommand{\cUtil}{\tilde{\cU}}
\newcommand{\cVtil}{\tilde{\cV}}
\newcommand{\cWtil}{\tilde{\cW}}
\newcommand{\cXtil}{\tilde{\cX}}
\newcommand{\cYtil}{\tilde{\cY}}
\newcommand{\cZtil}{\tilde{\cZ}}

\newcommand{\cAt}{\tilde{\cA}}
\newcommand{\cBt}{\tilde{\cB}}
\newcommand{\cCt}{\tilde{\cC}}
\newcommand{\cDt}{\tilde{\cD}}
\newcommand{\cEt}{\tilde{\cE}}
\newcommand{\cFt}{\tilde{\cF}}
\newcommand{\cGt}{\tilde{\cG}}
\newcommand{\cHt}{\tilde{\cH}}
\newcommand{\cIt}{\tilde{\cI}}
\newcommand{\cJt}{\tilde{\cJ}}
\newcommand{\cKt}{\tilde{\cK}}
\newcommand{\cLt}{\tilde{\cL}}
\newcommand{\cMt}{\tilde{\cM}}
\newcommand{\cNt}{\tilde{\cN}}
\newcommand{\cOt}{\tilde{\cO}}
\newcommand{\cPt}{\tilde{\cP}}
\newcommand{\cQt}{\tilde{\cQ}}
\newcommand{\cRt}{\tilde{\cR}}
\newcommand{\cSt}{\tilde{\cS}}
\newcommand{\cTt}{\tilde{\cT}}
\newcommand{\cUt}{\tilde{\cU}}
\newcommand{\cVt}{\tilde{\cV}}
\newcommand{\cWt}{\tilde{\cW}}
\newcommand{\cXt}{\tilde{\cX}}
\newcommand{\cYt}{\tilde{\cY}}
\newcommand{\cZt}{\tilde{\cZ}}

\newcommand{\cAtilde}{\widetilde{\cA}}
\newcommand{\cBtilde}{\widetilde{\cB}}
\newcommand{\cCtilde}{\widetilde{\cC}}
\newcommand{\cDtilde}{\widetilde{\cD}}
\newcommand{\cEtilde}{\widetilde{\cE}}
\newcommand{\cFtilde}{\widetilde{\cF}}
\newcommand{\cGtilde}{\widetilde{\cG}}
\newcommand{\cHtilde}{\widetilde{\cH}}
\newcommand{\cItilde}{\widetilde{\cI}}
\newcommand{\cJtilde}{\widetilde{\cJ}}
\newcommand{\cKtilde}{\widetilde{\cK}}
\newcommand{\cLtilde}{\widetilde{\cL}}
\newcommand{\cMtilde}{\widetilde{\cM}}
\newcommand{\cNtilde}{\widetilde{\cN}}
\newcommand{\cOtilde}{\widetilde{\cO}}
\newcommand{\cPtilde}{\widetilde{\cP}}
\newcommand{\cQtilde}{\widetilde{\cQ}}
\newcommand{\cRtilde}{\widetilde{\cR}}
\newcommand{\cStilde}{\widetilde{\cS}}
\newcommand{\cTtilde}{\widetilde{\cT}}
\newcommand{\cUtilde}{\widetilde{\cU}}
\newcommand{\cVtilde}{\widetilde{\cV}}
\newcommand{\cWtilde}{\widetilde{\cW}}
\newcommand{\cXtilde}{\widetilde{\cX}}
\newcommand{\cYtilde}{\widetilde{\cY}}
\newcommand{\cZtilde}{\widetilde{\cZ}}

\newcommand{\Acalhat}{\hat{\cA}}
\newcommand{\Bcalhat}{\hat{\cB}}
\newcommand{\Ccalhat}{\hat{\cC}}
\newcommand{\Dcalhat}{\hat{\cD}}
\newcommand{\Ecalhat}{\hat{\cE}}
\newcommand{\Fcalhat}{\hat{\cF}}
\newcommand{\Gcalhat}{\hat{\cG}}
\newcommand{\Hcalhat}{\hat{\cH}}
\newcommand{\Icalhat}{\hat{\cI}}
\newcommand{\Jcalhat}{\hat{\cJ}}
\newcommand{\Kcalhat}{\hat{\cK}}
\newcommand{\Lcalhat}{\hat{\cL}}
\newcommand{\Mcalhat}{\hat{\cM}}
\newcommand{\Ncalhat}{\hat{\cN}}
\newcommand{\Ocalhat}{\hat{\cO}}
\newcommand{\Pcalhat}{\hat{\cP}}
\newcommand{\Qcalhat}{\hat{\cQ}}
\newcommand{\Rcalhat}{\hat{\cR}}
\newcommand{\Scalhat}{\hat{\cS}}
\newcommand{\Tcalhat}{\hat{\cT}}
\newcommand{\Ucalhat}{\hat{\cU}}
\newcommand{\Vcalhat}{\hat{\cV}}
\newcommand{\Wcalhat}{\hat{\cW}}
\newcommand{\Xcalhat}{\hat{\cX}}
\newcommand{\Ycalhat}{\hat{\cY}}
\newcommand{\Zcalhat}{\hat{\cZ}}

\newcommand{\cAhat}{\hat{\cA}}
\newcommand{\cBhat}{\hat{\cB}}
\newcommand{\cChat}{\hat{\cC}}
\newcommand{\cDhat}{\hat{\cD}}
\newcommand{\cEhat}{\hat{\cE}}
\newcommand{\cFhat}{\hat{\cF}}
\newcommand{\cGhat}{\hat{\cG}}
\newcommand{\cHhat}{\hat{\cH}}
\newcommand{\cIhat}{\hat{\cI}}
\newcommand{\cJhat}{\hat{\cJ}}
\newcommand{\cKhat}{\hat{\cK}}
\newcommand{\cLhat}{\hat{\cL}}
\newcommand{\cMhat}{\hat{\cM}}
\newcommand{\cNhat}{\hat{\cN}}
\newcommand{\cOhat}{\hat{\cO}}
\newcommand{\cPhat}{\hat{\cP}}
\newcommand{\cQhat}{\hat{\cQ}}
\newcommand{\cRhat}{\hat{\cR}}
\newcommand{\cShat}{\hat{\cS}}
\newcommand{\cThat}{\hat{\cT}}
\newcommand{\cUhat}{\hat{\cU}}
\newcommand{\cVhat}{\hat{\cV}}
\newcommand{\cWhat}{\hat{\cW}}
\newcommand{\cXhat}{\hat{\cX}}
\newcommand{\cYhat}{\hat{\cY}}
\newcommand{\cZhat}{\hat{\cZ}}

\newcommand{\Acalbar}{\bar{\cA}}
\newcommand{\Bcalbar}{\bar{\cB}}
\newcommand{\Ccalbar}{\bar{\cC}}
\newcommand{\Dcalbar}{\bar{\cD}}
\newcommand{\Ecalbar}{\bar{\cE}}
\newcommand{\Fcalbar}{\bar{\cF}}
\newcommand{\Gcalbar}{\bar{\cG}}
\newcommand{\Hcalbar}{\bar{\cH}}
\newcommand{\Icalbar}{\bar{\cI}}
\newcommand{\Jcalbar}{\bar{\cJ}}
\newcommand{\Kcalbar}{\bar{\cK}}
\newcommand{\Lcalbar}{\bar{\cL}}
\newcommand{\Mcalbar}{\bar{\cM}}
\newcommand{\Ncalbar}{\bar{\cN}}
\newcommand{\Ocalbar}{\bar{\cO}}
\newcommand{\Pcalbar}{\bar{\cP}}
\newcommand{\Qcalbar}{\bar{\cQ}}
\newcommand{\Rcalbar}{\bar{\cR}}
\newcommand{\Scalbar}{\bar{\cS}}
\newcommand{\Tcalbar}{\bar{\cT}}
\newcommand{\Ucalbar}{\bar{\cU}}
\newcommand{\Vcalbar}{\bar{\cV}}
\newcommand{\Wcalbar}{\bar{\cW}}
\newcommand{\Xcalbar}{\bar{\cX}}
\newcommand{\Ycalbar}{\bar{\cY}}
\newcommand{\Zcalbar}{\bar{\cZ}}

\newcommand{\cAbar}{\bar{\cA}}
\newcommand{\cBbar}{\bar{\cB}}
\newcommand{\cCbar}{\bar{\cC}}
\newcommand{\cDbar}{\bar{\cD}}
\newcommand{\cEbar}{\bar{\cE}}
\newcommand{\cFbar}{\bar{\cF}}
\newcommand{\cGbar}{\bar{\cG}}
\newcommand{\cHbar}{\bar{\cH}}
\newcommand{\cIbar}{\bar{\cI}}
\newcommand{\cJbar}{\bar{\cJ}}
\newcommand{\cKbar}{\bar{\cK}}
\newcommand{\cLbar}{\bar{\cL}}
\newcommand{\cMbar}{\bar{\cM}}
\newcommand{\cNbar}{\bar{\cN}}
\newcommand{\cObar}{\bar{\cO}}
\newcommand{\cPbar}{\bar{\cP}}
\newcommand{\cQbar}{\bar{\cQ}}
\newcommand{\cRbar}{\bar{\cR}}
\newcommand{\cSbar}{\bar{\cS}}
\newcommand{\cTbar}{\bar{\cT}}
\newcommand{\cUbar}{\bar{\cU}}
\newcommand{\cVbar}{\bar{\cV}}
\newcommand{\cWbar}{\bar{\cW}}
\newcommand{\cXbar}{\bar{\cX}}
\newcommand{\cYbar}{\bar{\cY}}
\newcommand{\cZbar}{\bar{\cZ}}

% mathscr version
\newcommand{\sA}{\mathscr{A}}
\newcommand{\sB}{\mathscr{B}}
\newcommand{\sC}{\mathscr{C}}
\newcommand{\sD}{\mathscr{D}}
\newcommand{\sE}{\mathscr{E}}
\newcommand{\sF}{\mathscr{F}}
\newcommand{\sG}{\mathscr{G}}
\newcommand{\sH}{\mathscr{H}}
\newcommand{\sI}{\mathscr{I}}
\newcommand{\sJ}{\mathscr{J}}
\newcommand{\sK}{\mathscr{K}}
\newcommand{\sL}{\mathscr{L}}
\newcommand{\sM}{\mathscr{M}}
\newcommand{\sN}{\mathscr{N}}
\newcommand{\sO}{\mathscr{O}}
\newcommand{\sP}{\mathscr{P}}
\newcommand{\sQ}{\mathscr{Q}}
\newcommand{\sR}{\mathscr{R}}
\newcommand{\sS}{\mathscr{S}}
\newcommand{\sT}{\mathscr{T}}
\newcommand{\sU}{\mathscr{U}}
\newcommand{\sV}{\mathscr{V}}
\newcommand{\sW}{\mathscr{W}}
\newcommand{\sX}{\mathscr{X}}
\newcommand{\sY}{\mathscr{Y}}
\newcommand{\sZ}{\mathscr{Z}}

\newcommand{\sAbar}{\bar{\sA}}
\newcommand{\sBbar}{\bar{\sB}}
\newcommand{\sCbar}{\bar{\sC}}
\newcommand{\sDbar}{\bar{\sD}}
\newcommand{\sEbar}{\bar{\sE}}
\newcommand{\sFbar}{\bar{\sF}}
\newcommand{\sGbar}{\bar{\sG}}
\newcommand{\sHbar}{\bar{\sH}}
\newcommand{\sIbar}{\bar{\sI}}
\newcommand{\sJbar}{\bar{\sJ}}
\newcommand{\sKbar}{\bar{\sK}}
\newcommand{\sLbar}{\bar{\sL}}
\newcommand{\sMbar}{\bar{\sM}}
\newcommand{\sNbar}{\bar{\sN}}
\newcommand{\sObar}{\bar{\sO}}
\newcommand{\sPbar}{\bar{\sP}}
\newcommand{\sQbar}{\bar{\sQ}}
\newcommand{\sRbar}{\bar{\sR}}
\newcommand{\sSbar}{\bar{\sS}}
\newcommand{\sTbar}{\bar{\sT}}
\newcommand{\sUbar}{\bar{\sU}}
\newcommand{\sVbar}{\bar{\sV}}
\newcommand{\sWbar}{\bar{\sW}}
\newcommand{\sXbar}{\bar{\sX}}
\newcommand{\sYbar}{\bar{\sY}}
\newcommand{\sZbar}{\bar{\sZ}}

\newcommand{\sAhat}{\hat{\sA}}
\newcommand{\sBhat}{\hat{\sB}}
\newcommand{\sChat}{\hat{\sC}}
\newcommand{\sDhat}{\hat{\sD}}
\newcommand{\sEhat}{\hat{\sE}}
\newcommand{\sFhat}{\hat{\sF}}
\newcommand{\sGhat}{\hat{\sG}}
\newcommand{\sHhat}{\hat{\sH}}
\newcommand{\sIhat}{\hat{\sI}}
\newcommand{\sJhat}{\hat{\sJ}}
\newcommand{\sKhat}{\hat{\sK}}
\newcommand{\sLhat}{\hat{\sL}}
\newcommand{\sMhat}{\hat{\sM}}
\newcommand{\sNhat}{\hat{\sN}}
\newcommand{\sOhat}{\hat{\sO}}
\newcommand{\sPhat}{\hat{\sP}}
\newcommand{\sQhat}{\hat{\sQ}}
\newcommand{\sRhat}{\hat{\sR}}
\newcommand{\sShat}{\hat{\sS}}
\newcommand{\sThat}{\hat{\sT}}
\newcommand{\sUhat}{\hat{\sU}}
\newcommand{\sVhat}{\hat{\sV}}
\newcommand{\sWhat}{\hat{\sW}}
\newcommand{\sXhat}{\hat{\sX}}
\newcommand{\sYhat}{\hat{\sY}}
\newcommand{\sZhat}{\hat{\sZ}}

\newcommand{\sAtilde}{\widetilde{\sA}}
\newcommand{\sBtilde}{\widetilde{\sB}}
\newcommand{\sCtilde}{\widetilde{\sC}}
\newcommand{\sDtilde}{\widetilde{\sD}}
\newcommand{\sEtilde}{\widetilde{\sE}}
\newcommand{\sFtilde}{\widetilde{\sF}}
\newcommand{\sGtilde}{\widetilde{\sG}}
\newcommand{\sHtilde}{\widetilde{\sH}}
\newcommand{\sItilde}{\widetilde{\sI}}
\newcommand{\sJtilde}{\widetilde{\sJ}}
\newcommand{\sKtilde}{\widetilde{\sK}}
\newcommand{\sLtilde}{\widetilde{\sL}}
\newcommand{\sMtilde}{\widetilde{\sM}}
\newcommand{\sNtilde}{\widetilde{\sN}}
\newcommand{\sOtilde}{\widetilde{\sO}}
\newcommand{\sPtilde}{\widetilde{\sP}}
\newcommand{\sQtilde}{\widetilde{\sQ}}
\newcommand{\sRtilde}{\widetilde{\sR}}
\newcommand{\sStilde}{\widetilde{\sS}}
\newcommand{\sTtilde}{\widetilde{\sT}}
\newcommand{\sUtilde}{\widetilde{\sU}}
\newcommand{\sVtilde}{\widetilde{\sV}}
\newcommand{\sWtilde}{\widetilde{\sW}}
\newcommand{\sXtilde}{\widetilde{\sX}}
\newcommand{\sYtilde}{\widetilde{\sY}}
\newcommand{\sZtilde}{\widetilde{\sZ}}

\newcommand{\sAt}{\tilde{\sA}}
\newcommand{\sBt}{\tilde{\sB}}
\newcommand{\sCt}{\tilde{\sC}}
\newcommand{\sDt}{\tilde{\sD}}
\newcommand{\sEt}{\tilde{\sE}}
\newcommand{\sFt}{\tilde{\sF}}
\newcommand{\sGt}{\tilde{\sG}}
\newcommand{\sHt}{\tilde{\sH}}
\newcommand{\sIt}{\tilde{\sI}}
\newcommand{\sJt}{\tilde{\sJ}}
\newcommand{\sKt}{\tilde{\sK}}
\newcommand{\sLt}{\tilde{\sL}}
\newcommand{\sMt}{\tilde{\sM}}
\newcommand{\sNt}{\tilde{\sN}}
\newcommand{\sOt}{\tilde{\sO}}
\newcommand{\sPt}{\tilde{\sP}}
\newcommand{\sQt}{\tilde{\sQ}}
\newcommand{\sRt}{\tilde{\sR}}
\newcommand{\sSt}{\tilde{\sS}}
\newcommand{\sTt}{\tilde{\sT}}
\newcommand{\sUt}{\tilde{\sU}}
\newcommand{\sVt}{\tilde{\sV}}
\newcommand{\sWt}{\tilde{\sW}}
\newcommand{\sXt}{\tilde{\sX}}
\newcommand{\sYt}{\tilde{\sY}}
\newcommand{\sZt}{\tilde{\sZ}}

% mathds version
\newcommand{\dA}{\mathds{A}}
\newcommand{\dB}{\mathds{B}}
\newcommand{\dC}{\mathds{C}}
\newcommand{\dD}{\mathds{D}}
\newcommand{\dE}{\mathds{E}}
\newcommand{\dF}{\mathds{F}}
\newcommand{\dG}{\mathds{G}}
\newcommand{\dH}{\mathds{H}}
\newcommand{\dI}{\mathds{I}}
\newcommand{\dJ}{\mathds{J}}
\newcommand{\dK}{\mathds{K}}
\newcommand{\dL}{\mathds{L}}
\newcommand{\dM}{\mathds{M}}
\newcommand{\dN}{\mathds{N}}
\newcommand{\dO}{\mathds{O}}
\newcommand{\dP}{\mathds{P}}
\newcommand{\dQ}{\mathds{Q}}
\newcommand{\dR}{\mathds{R}}
\newcommand{\dS}{\mathds{S}}
\newcommand{\dT}{\mathds{T}}
\newcommand{\dU}{\mathds{U}}
\newcommand{\dV}{\mathds{V}}
\newcommand{\dW}{\mathds{W}}
\newcommand{\dX}{\mathds{X}}
\newcommand{\dY}{\mathds{Y}}
\newcommand{\dZ}{\mathds{Z}}

\newcommand{\dAbar}{\bar{\dA}}
\newcommand{\dBbar}{\bar{\dB}}
\newcommand{\dCbar}{\bar{\dC}}
\newcommand{\dDbar}{\bar{\dD}}
\newcommand{\dEbar}{\bar{\dE}}
\newcommand{\dFbar}{\bar{\dF}}
\newcommand{\dGbar}{\bar{\dG}}
\newcommand{\dHbar}{\bar{\dH}}
\newcommand{\dIbar}{\bar{\dI}}
\newcommand{\dJbar}{\bar{\dJ}}
\newcommand{\dKbar}{\bar{\dK}}
\newcommand{\dLbar}{\bar{\dL}}
\newcommand{\dMbar}{\bar{\dM}}
\newcommand{\dNbar}{\bar{\dN}}
\newcommand{\dObar}{\bar{\dO}}
\newcommand{\dPbar}{\bar{\dP}}
\newcommand{\dQbar}{\bar{\dQ}}
\newcommand{\dRbar}{\bar{\dR}}
\newcommand{\dSbar}{\bar{\dS}}
\newcommand{\dTbar}{\bar{\dT}}
\newcommand{\dUbar}{\bar{\dU}}
\newcommand{\dVbar}{\bar{\dV}}
\newcommand{\dWbar}{\bar{\dW}}
\newcommand{\dXbar}{\bar{\dX}}
\newcommand{\dYbar}{\bar{\dY}}
\newcommand{\dZbar}{\bar{\dZ}}

\newcommand{\dAhat}{\hat{\dA}}
\newcommand{\dBhat}{\hat{\dB}}
\newcommand{\dChat}{\hat{\dC}}
\newcommand{\dDhat}{\hat{\dD}}
\newcommand{\dEhat}{\hat{\dE}}
\newcommand{\dFhat}{\hat{\dF}}
\newcommand{\dGhat}{\hat{\dG}}
\newcommand{\dHhat}{\hat{\dH}}
\newcommand{\dIhat}{\hat{\dI}}
\newcommand{\dJhat}{\hat{\dJ}}
\newcommand{\dKhat}{\hat{\dK}}
\newcommand{\dLhat}{\hat{\dL}}
\newcommand{\dMhat}{\hat{\dM}}
\newcommand{\dNhat}{\hat{\dN}}
\newcommand{\dOhat}{\hat{\dO}}
\newcommand{\dPhat}{\hat{\dP}}
\newcommand{\dQhat}{\hat{\dQ}}
\newcommand{\dRhat}{\hat{\dR}}
\newcommand{\dShat}{\hat{\dS}}
\newcommand{\dThat}{\hat{\dT}}
\newcommand{\dUhat}{\hat{\dU}}
\newcommand{\dVhat}{\hat{\dV}}
\newcommand{\dWhat}{\hat{\dW}}
\newcommand{\dXhat}{\hat{\dX}}
\newcommand{\dYhat}{\hat{\dY}}
\newcommand{\dZhat}{\hat{\dZ}}

\newcommand{\dAtilde}{\widetilde{\dA}}
\newcommand{\dBtilde}{\widetilde{\dB}}
\newcommand{\dCtilde}{\widetilde{\dC}}
\newcommand{\dDtilde}{\widetilde{\dD}}
\newcommand{\dEtilde}{\widetilde{\dE}}
\newcommand{\dFtilde}{\widetilde{\dF}}
\newcommand{\dGtilde}{\widetilde{\dG}}
\newcommand{\dHtilde}{\widetilde{\dH}}
\newcommand{\dItilde}{\widetilde{\dI}}
\newcommand{\dJtilde}{\widetilde{\dJ}}
\newcommand{\dKtilde}{\widetilde{\dK}}
\newcommand{\dLtilde}{\widetilde{\dL}}
\newcommand{\dMtilde}{\widetilde{\dM}}
\newcommand{\dNtilde}{\widetilde{\dN}}
\newcommand{\dOtilde}{\widetilde{\dO}}
\newcommand{\dPtilde}{\widetilde{\dP}}
\newcommand{\dQtilde}{\widetilde{\dQ}}
\newcommand{\dRtilde}{\widetilde{\dR}}
\newcommand{\dStilde}{\widetilde{\dS}}
\newcommand{\dTtilde}{\widetilde{\dT}}
\newcommand{\dUtilde}{\widetilde{\dU}}
\newcommand{\dVtilde}{\widetilde{\dV}}
\newcommand{\dWtilde}{\widetilde{\dW}}
\newcommand{\dXtilde}{\widetilde{\dX}}
\newcommand{\dYtilde}{\widetilde{\dY}}
\newcommand{\dZtilde}{\widetilde{\dZ}}

\newcommand{\dAt}{\tilde{\dA}}
\newcommand{\dBt}{\tilde{\dB}}
\newcommand{\dCt}{\tilde{\dC}}
\newcommand{\dDt}{\tilde{\dD}}
\newcommand{\dEt}{\tilde{\dE}}
\newcommand{\dFt}{\tilde{\dF}}
\newcommand{\dGt}{\tilde{\dG}}
\newcommand{\dHt}{\tilde{\dH}}
\newcommand{\dIt}{\tilde{\dI}}
\newcommand{\dJt}{\tilde{\dJ}}
\newcommand{\dKt}{\tilde{\dK}}
\newcommand{\dLt}{\tilde{\dL}}
\newcommand{\dMt}{\tilde{\dM}}
\newcommand{\dNt}{\tilde{\dN}}
\newcommand{\dOt}{\tilde{\dO}}
\newcommand{\dPt}{\tilde{\dP}}
\newcommand{\dQt}{\tilde{\dQ}}
\newcommand{\dRt}{\tilde{\dR}}
\newcommand{\dSt}{\tilde{\dS}}
\newcommand{\dTt}{\tilde{\dT}}
\newcommand{\dUt}{\tilde{\dU}}
\newcommand{\dVt}{\tilde{\dV}}
\newcommand{\dWt}{\tilde{\dW}}
\newcommand{\dXt}{\tilde{\dX}}
\newcommand{\dYt}{\tilde{\dY}}
\newcommand{\dZt}{\tilde{\dZ}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\ve}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vj}{\vec{j}}
\newcommand{\vk}{\vec{k}}
\newcommand{\vl}{\vec{l}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vn}{\vec{n}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\Proof\undefined
\newcommand{\Proof}{\noindent{\bf Proof.}~}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{lemma}{Lemma}
\fi

\ifx\proposition\undefined
%\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
%\newtheorem{remark}[theorem]{Remark}
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
%\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

\ifx\claim\undefined
%\newtheorem{claim}[theorem]{Claim}
\newtheorem{claim}{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\done}{\mathds{1}} % Indicator with 1
\newcommand{\dAA}{\mathds{A}} 
\newcommand{\BB}{\mathds{B}} 
\newcommand{\CC}{\mathds{C}} % Complex numbers
\newcommand{\DD}{\mathds{D}} 
\newcommand{\EE}{\mathds{E}} % Expectation
\newcommand{\FF}{\mathds{F}} % Fexpectation
\newcommand{\GG}{\mathds{G}} 
\newcommand{\HH}{\mathds{H}} % Arbitrary field
\newcommand{\II}{\mathds{I}} % Delta Indicator with I
\newcommand{\JJ}{\mathds{J}} 
\newcommand{\KK}{\mathds{K}} % Arbitrary field
\newcommand{\LL}{\mathds{L}} 
\newcommand{\MM}{\mathds{M}} % Median
\newcommand{\NN}{\mathds{N}} % Natural numbers
\newcommand{\OO}{\mathds{O}} 
\newcommand{\PP}{\mathds{P}} % Probability
\newcommand{\QQ}{\mathds{Q}} % Rationals
\newcommand{\RR}{\mathds{R}} % Real numbers
\newcommand{\dSS}{\mathbb{S}} 
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\TT}{\mathds{T}} 
\newcommand{\UU}{\mathds{U}} 
\newcommand{\VV}{\mathds{V}} % Variance
\newcommand{\WW}{\mathds{W}} 
\newcommand{\XX}{\mathds{X}}
\newcommand{\YY}{\mathds{Y}}
\newcommand{\ZZ}{\mathds{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\operatorname*{minimize}}
\newcommand*{\maxi}{\operatorname*{maximize}}
\newcommand*{\argmin}{\operatorname*{argmin}}
\newcommand*{\argmax}{\operatorname*{argmax}}
\newcommand*{\arginf}{\operatorname*{arginf}}
\newcommand*{\argsup}{\operatorname*{argsup}}

\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

% version with default argument: e.g., \diag => diag ; \diag[A] => diag(A)
\newcommand{\co}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{co}\else\operatorname{co}\left(#1\right)\fi}
\newcommand{\core}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{core}\else\operatorname{core}\left(#1\right)\fi}
\newcommand{\diag}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{diag}\else\operatorname{diag}\left(#1\right)\fi}
\newcommand{\dom}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{dom}\else\operatorname{dom}\left(#1\right)\fi}
\newcommand{\expect}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{E}}\else\operatorname{\mathds{E}}\ssbr{#1}\fi}
\newcommand{\ind}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{I}}\else\operatorname{\mathds{I}}\left[#1\right]\fi}
\newcommand{\lap}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\bf Lap}\else\operatorname{\bf Lap}\left(#1\right)\fi}
\newcommand{\prob}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{P}}\else\operatorname{\mathds{P}}\ssbr{#1}\fi}
\newcommand{\proj}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathcal{P}}\else\operatorname{\mathcal{P}}\left(#1\right)\fi}
\newcommand{\prox}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{prox}\else\operatorname{prox}\left(#1\right)\fi}
\newcommand{\rank}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{rank}\else\operatorname{rank}\left(#1\right)\fi}
\newcommand{\sgn}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{sign}\else\operatorname{sign}\left(#1\right)\fi}
\newcommand{\sign}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{sign}\else\operatorname{sign}\left(#1\right)\fi}
\newcommand{\tr}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{tr}\else\operatorname{tr}\left(#1\right)\fi}
\newcommand{\trace}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{tr}\else\operatorname{tr}\left(#1\right)\fi}
\newcommand{\traj}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{Traj}\else\operatorname{Traj}\left(#1\right)\fi}
\newcommand{\var}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{\mathds{V}}\else\operatorname{\mathds{V}}\left[#1\right]\fi}
\newcommand{\vect}[1][]{\def\tst{#1}\ifx\tst\empty\operatorname{vec}\else\operatorname{vec}\left(#1\right)\fi}

\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\ri}{\operatorname{ri}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\intr}{\operatorname{int}}
%\newcommand{\bd}{\operatorname{bd}}
\newcommand{\emp}{\operatorname{emp}}
\newcommand{\nnz}{\operatorname{nnz}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}
\renewcommand{\O}{{\cO}}
\newcommand{\softO}[1]{{\widetilde{\cO}}\rbr{#1}}

% version with argument
\newcommand{\Co}[1]{\co[#1]}
\newcommand{\Core}[1]{\core[#1]}
\newcommand{\Diag}[1]{\diag[#1]}
\newcommand{\Dom}[1]{\dom[#1]}
\newcommand{\Expect}[2][]{\underset{#1}{\EE}\ssbr{{#2}}}
\newcommand{\Ind}[1]{\ind[#1]}
\newcommand{\Lap}[1]{\lap[#1]}
\newcommand{\Prob}[1]{\prob[#1]}
\newcommand{\Proj}[2][]{\mathcal{P}_{#1}\sbr{#2}}
\newcommand{\Prox}[2][]{\operatorname{prox}_{#1}\rbr{#2}}
\newcommand{\Rank}[1]{\rank[#1]}
\newcommand{\Sgn}[1]{\sgn[#1]}
\newcommand{\Sign}[1]{\sign[#1]}
\newcommand{\Tr}[1]{\trace[#1]}
\newcommand{\Trace}[1]{\trace[#1]}
\newcommand{\Traj}[1]{\traj[#1]}
\newcommand{\Var}[1]{\var[#1]}
\newcommand{\Vect}[1]{\vect[#1]}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}


\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}

%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left({#1}\right)}
\newcommand{\sbr}[1]{\left[{#1}\right]}
\newcommand{\cbr}[1]{\left\{{#1}\right\}}
\newcommand{\nbr}[1]{\left\|{#1}\right\|}
\newcommand{\abr}[1]{\left\langle{#1}\right\rangle}
\newcommand{\abs}[1]{\left|{#1}\right|}
\newcommand{\floor}[1]{\left\lfloor {#1} \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil {#1} \right\rceil}
\newcommand{\inner}[2]{\left\langle {#1},{#2} \right\rangle}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\frob}[1]{\norm{#1}_\text{F}}
\newcommand{\fro}[1]{\norm{#1}_\text{F}}
\newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\twonorm}[1]{\norm{#1}_2}
\newcommand{\infnorm}[1]{\norm{#1}_{\infty}}
\newcommand{\trnorm}[1]{\norm{#1}_{\text{tr}}}
\newcommand{\ccc}[1]{\left|\!\left|\!\left|{#1}\right|\!\right|\!\right|}
\newcommand{\bsd}[1]{\left\llbracket{#1}\right\rrbracket}
\newcommand{\ssbr}[1]{\left\llbracket{#1}\right\rrbracket}
\newcommand{\sembrack}[1]{\left\llbracket{#1}\right\rrbracket}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{{\bm{1}}}  % Identity
\newcommand{\zero}{{\bm{0}}} % Zero
\newcommand{\bone}{{\bm{1}}}  % Identity
\newcommand{\bzero}{{\bm{0}}} % Zero
\def\b0{\bm{0}} % Zero
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}
\newcommand*{\diff}[1][]{\mathop{}\!{\mathrm{d}^{#1}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\valpha}{\vec{\alpha}}
\newcommand{\AL}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vgamma}{\vec{\gamma}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vdelta}{\vec{\delta}}
\newcommand{\veps}{\vec{\epsilon}}
\newcommand{\vepsilon}{\vec{\epsilon}}
\newcommand{\vze}{\vec{\zeta}}
\newcommand{\vzeta}{\vec{\zeta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\vtheta}{\vec{\theta}}
\newcommand{\viota}{\vec{\iota}}
\newcommand{\vkappa}{\vec{\kappa}}
\newcommand{\vlambda}{\vec{\lambda}}
\newcommand{\vmu}{\vec{\mu}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vrho}{\vec{\rho}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\vupsilon}{\vec{\upsilon}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vchi}{\vec{\chi}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vomega}{\vec{\omega}}

\newcommand{\bal}{\vec{\alpha}}
\newcommand{\balpha}{\vec{\alpha}}
\newcommand{\bbeta}{\vec{\beta}}
\newcommand{\bga}{\vec{\gamma}}
\newcommand{\bgamma}{\vec{\gamma}}
\newcommand{\bde}{\vec{\delta}}
\newcommand{\bdelta}{\vec{\delta}}
\newcommand{\beps}{\vec{\epsilon}}
\newcommand{\bepsilon}{\vec{\epsilon}}
\newcommand{\bze}{\vec{\zeta}}
\newcommand{\bzeta}{\vec{\zeta}}
\newcommand{\boldeta}{\vec{\eta}}
\newcommand{\bth}{\vec{\theta}}
\newcommand{\btheta}{\vec{\theta}}
\newcommand{\biota}{\vec{\iota}}
\newcommand{\bkappa}{\vec{\kappa}}
\newcommand{\blambda}{\vec{\lambda}}
\newcommand{\bmu}{\vec{\mu}}
\newcommand{\bnu}{\vec{\nu}}
\newcommand{\bxi}{\vec{\xi}}
\newcommand{\bpi}{\vec{\pi}}
\newcommand{\brho}{\vec{\rho}}
\newcommand{\bsig}{\vec{\sigma}}
\newcommand{\bsigma}{\vec{\sigma}}
\newcommand{\btau}{\vec{\tau}}
\newcommand{\bupsilon}{\vec{\upsilon}}
\newcommand{\bphi}{\vec{\phi}}
\newcommand{\bchi}{\vec{\chi}}
\newcommand{\bpsi}{\vec{\psi}}
\newcommand{\bomega}{\vec{\omega}}

\newcommand{\ALbar}{\bar{\val}}
\newcommand{\balbar}{\bar{\val}}
\newcommand{\balphabar}{\bar{\val}}
\newcommand{\bbetabar}{\bar{\vbeta}}
\newcommand{\bgabar}{\bar{\vgamma}}
\newcommand{\bgammabar}{\bar{\vgamma}}
\newcommand{\bdebar}{\bar{\vdelta}}
\newcommand{\bdeltabar}{\bar{\vdelta}}
\newcommand{\bepsbar}{\bar{\vepsilon}}
\newcommand{\bepsilonbar}{\bar{\vepsilon}}
\newcommand{\bzebar}{\bar{\vzeta}}
\newcommand{\bzetabar}{\bar{\vzeta}}
\newcommand{\boldetabar}{\bar{\veta}}
\newcommand{\bthbar}{\bar{\vtheta}}
\newcommand{\bthetabar}{\bar{\vtheta}}
\newcommand{\biotabar}{\bar{\viota}}
\newcommand{\bkappabar}{\bar{\vkappa}}
\newcommand{\blambdabar}{\bar{\vlambda}}
\newcommand{\bmubar}{\bar{\vmu}}
\newcommand{\bnubar}{\bar{\vnu}}
\newcommand{\bxibar}{\bar{\vxi}}
\newcommand{\bpibar}{\bar{\vpi}}
\newcommand{\brhobar}{\bar{\vrho}}
\newcommand{\bsigbar}{\bar{\vsigma}}
\newcommand{\bsigmabar}{\bar{\vsigma}}
\newcommand{\btaubar}{\bar{\vtau}}
\newcommand{\bupsilonbar}{\bar{\vupsilon}}
\newcommand{\bphibar}{\bar{\vphi}}
\newcommand{\bchibar}{\bar{\vchi}}
\newcommand{\bpsibar}{\bar{\vpsi}}
\newcommand{\bomegabar}{\bar{\vomega}}

\newcommand{\ALhat}{\hat{\val}}
\newcommand{\balhat}{\hat{\val}}
\newcommand{\balphahat}{\hat{\val}}
\newcommand{\bbetahat}{\hat{\vbeta}}
\newcommand{\bgahat}{\hat{\vgamma}}
\newcommand{\bgammahat}{\hat{\vgamma}}
\newcommand{\bdehat}{\hat{\vdelta}}
\newcommand{\bdeltahat}{\hat{\vdelta}}
\newcommand{\bepshat}{\hat{\vepsilon}}
\newcommand{\bepsilonhat}{\hat{\vepsilon}}
\newcommand{\bzehat}{\hat{\vzeta}}
\newcommand{\bzetahat}{\hat{\vzeta}}
\newcommand{\boldetahat}{\hat{\veta}}
\newcommand{\bthhat}{\hat{\vtheta}}
\newcommand{\bthetahat}{\hat{\vtheta}}
\newcommand{\biotahat}{\hat{\viota}}
\newcommand{\bkappahat}{\hat{\vkappa}}
\newcommand{\blambdahat}{\hat{\vlambda}}
\newcommand{\bmuhat}{\hat{\vmu}}
\newcommand{\bnuhat}{\hat{\vnu}}
\newcommand{\bxihat}{\hat{\vxi}}
\newcommand{\bpihat}{\hat{\vpi}}
\newcommand{\brhohat}{\hat{\vrho}}
\newcommand{\bsighat}{\hat{\vsigma}}
\newcommand{\bsigmahat}{\hat{\vsigma}}
\newcommand{\btauhat}{\hat{\vtau}}
\newcommand{\bupsilonhat}{\hat{\vupsilon}}
\newcommand{\bphihat}{\hat{\vphi}}
\newcommand{\bchihat}{\hat{\vchi}}
\newcommand{\bpsihat}{\hat{\vpsi}}
\newcommand{\bomegahat}{\hat{\vomega}}

\newcommand{\ALtil}{\tilde{\val}}
\newcommand{\baltil}{\tilde{\val}}
\newcommand{\balphatil}{\tilde{\val}}
\newcommand{\bbetatil}{\tilde{\vbeta}}
\newcommand{\bgatil}{\tilde{\vgamma}}
\newcommand{\bgammatil}{\tilde{\vgamma}}
\newcommand{\bdetil}{\tilde{\vdelta}}
\newcommand{\bdeltatil}{\tilde{\vdelta}}
\newcommand{\bepstil}{\tilde{\vepsilon}}
\newcommand{\bepsilontil}{\tilde{\vepsilon}}
\newcommand{\bzetil}{\tilde{\vzeta}}
\newcommand{\bzetatil}{\tilde{\vzeta}}
\newcommand{\boldetatil}{\tilde{\veta}}
\newcommand{\bthtil}{\tilde{\vtheta}}
\newcommand{\bthetatil}{\tilde{\vtheta}}
\newcommand{\biotatil}{\tilde{\viota}}
\newcommand{\bkappatil}{\tilde{\vkappa}}
\newcommand{\blambdatil}{\tilde{\vlambda}}
\newcommand{\bmutil}{\tilde{\vmu}}
\newcommand{\bnutil}{\tilde{\vnu}}
\newcommand{\bxitil}{\tilde{\vxi}}
\newcommand{\bpitil}{\tilde{\vpi}}
\newcommand{\brhotil}{\tilde{\vrho}}
\newcommand{\bsigtil}{\tilde{\vsigma}}
\newcommand{\bsigmatil}{\tilde{\vsigma}}
\newcommand{\btautil}{\tilde{\vtau}}
\newcommand{\bupsilontil}{\tilde{\vupsilon}}
\newcommand{\bphitil}{\tilde{\vphi}}
\newcommand{\bchitil}{\tilde{\vchi}}
\newcommand{\bpsitil}{\tilde{\vpsi}}
\newcommand{\bomegatil}{\tilde{\vomega}}

\newcommand{\ALtilde}{\widetilde{\val}}
\newcommand{\baltilde}{\widetilde{\val}}
\newcommand{\balphatilde}{\widetilde{\val}}
\newcommand{\bbetatilde}{\widetilde{\vbeta}}
\newcommand{\bgatilde}{\widetilde{\vgamma}}
\newcommand{\bgammatilde}{\widetilde{\vgamma}}
\newcommand{\bdetilde}{\widetilde{\vdelta}}
\newcommand{\bdeltatilde}{\widetilde{\vdelta}}
\newcommand{\bepstilde}{\widetilde{\vepsilon}}
\newcommand{\bepsilontilde}{\widetilde{\vepsilon}}
\newcommand{\bzetilde}{\widetilde{\vzeta}}
\newcommand{\bzetatilde}{\widetilde{\vzeta}}
\newcommand{\boldetatilde}{\widetilde{\veta}}
\newcommand{\bthtilde}{\widetilde{\vtheta}}
\newcommand{\bthetatilde}{\widetilde{\vtheta}}
\newcommand{\biotatilde}{\widetilde{\viota}}
\newcommand{\bkappatilde}{\widetilde{\vkappa}}
\newcommand{\blambdatilde}{\widetilde{\vlambda}}
\newcommand{\bmutilde}{\widetilde{\vmu}}
\newcommand{\bnutilde}{\widetilde{\vnu}}
\newcommand{\bxitilde}{\widetilde{\vxi}}
\newcommand{\bpitilde}{\widetilde{\vpi}}
\newcommand{\brhotilde}{\widetilde{\vrho}}
\newcommand{\bsigtilde}{\widetilde{\vsigma}}
\newcommand{\bsigmatilde}{\widetilde{\vsigma}}
\newcommand{\btautilde}{\widetilde{\vtau}}
\newcommand{\bupsilontilde}{\widetilde{\vupsilon}}
\newcommand{\bphitilde}{\widetilde{\vphi}}
\newcommand{\bchitilde}{\widetilde{\vchi}}
\newcommand{\bpsitilde}{\widetilde{\vpsi}}
\newcommand{\bomegatilde}{\widetilde{\vomega}}

\newcommand{\ALt}{\tilde{\val}}
\newcommand{\balt}{\tilde{\val}}
\newcommand{\balphat}{\hat{\val}}
\newcommand{\bbetat}{\tilde{\vbeta}}
\newcommand{\bgat}{\tilde{\vgamma}}
\newcommand{\bgammat}{\tilde{\vgamma}}
\newcommand{\bdet}{\tilde{\vdelta}}
\newcommand{\bdeltat}{\tilde{\vdelta}}
\newcommand{\bepst}{\tilde{\vepsilon}}
\newcommand{\bepsilont}{\tilde{\vepsilon}}
\newcommand{\bzet}{\tilde{\vzeta}}
\newcommand{\bzetat}{\tilde{\vzeta}}
\newcommand{\boldetat}{\tilde{\veta}}
\newcommand{\btht}{\tilde{\vtheta}}
\newcommand{\bthetat}{\tilde{\vtheta}}
\newcommand{\biotat}{\tilde{\viota}}
\newcommand{\bkappat}{\tilde{\vkappa}}
\newcommand{\blambdat}{\tilde{\vlambda}}
\newcommand{\bmut}{\tilde{\vmu}}
\newcommand{\bnut}{\tilde{\vnu}}
\newcommand{\bxit}{\tilde{\vxi}}
\newcommand{\bpit}{\tilde{\vpi}}
\newcommand{\brhot}{\tilde{\vrho}}
\newcommand{\bsigt}{\tilde{\vsigma}}
\newcommand{\bsigmat}{\tilde{\vsigma}}
\newcommand{\btaut}{\tilde{\vtau}}
\newcommand{\bupsilont}{\tilde{\vupsilon}}
\newcommand{\bphit}{\tilde{\vphi}}
\newcommand{\bchit}{\tilde{\vchi}}
\newcommand{\bpsit}{\tilde{\vpsi}}
\newcommand{\bomegat}{\tilde{\vomega}}

\newcommand{\albar}{\bar{\al}}
\newcommand{\alphabar}{\bar{\al}}
\newcommand{\betabar}{\bar{\beta}}
\newcommand{\gabar}{\bar{\gamma}}
\newcommand{\gammabar}{\bar{\gamma}}
\newcommand{\debar}{\bar{\delta}}
\newcommand{\deltabar}{\bar{\delta}}
\newcommand{\epsbar}{\bar{\epsilon}}
\newcommand{\epsilonbar}{\bar{\epsilon}}
\newcommand{\zebar}{\bar{\zeta}}
\newcommand{\zetabar}{\bar{\zeta}}
\newcommand{\etabar}{\bar{\eta}}
\newcommand{\thbar}{\bar{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\iotabar}{\bar{\iota}}
\newcommand{\kappabar}{\bar{\kappa}}
\newcommand{\lambdabar}{\bar{\lambda}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\nubar}{\bar{\nu}}
\newcommand{\xibar}{\bar{\xi}}
\newcommand{\pibar}{\bar{\pi}}
\newcommand{\rhobar}{\bar{\rho}}
\newcommand{\sigbar}{\bar{\sigma}}
\newcommand{\sigmabar}{\bar{\sigma}}
\newcommand{\taubar}{\bar{\tau}}
\newcommand{\upsilonbar}{\bar{\upsilon}}
\newcommand{\phibar}{\bar{\phi}}
\newcommand{\chibar}{\bar{\chi}}
\newcommand{\psibar}{\bar{\psi}}
\newcommand{\omegabar}{\bar{\omega}}

\newcommand{\alhat}{\hat{\al}}
\newcommand{\alphahat}{\hat{\al}}
\newcommand{\betahat}{\hat{\beta}}
\newcommand{\gahat}{\hat{\gamma}}
\newcommand{\gammahat}{\hat{\gamma}}
\newcommand{\dehat}{\hat{\delta}}
\newcommand{\deltahat}{\hat{\delta}}
\newcommand{\epshat}{\hat{\epsilon}}
\newcommand{\epsilonhat}{\hat{\epsilon}}
\newcommand{\zehat}{\hat{\zeta}}
\newcommand{\zetahat}{\hat{\zeta}}
\newcommand{\etahat}{\hat{\eta}}
\newcommand{\thhat}{\hat{\theta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\iotahat}{\hat{\iota}}
\newcommand{\kappahat}{\hat{\kappa}}
\newcommand{\lambdahat}{\hat{\lambda}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\nuhat}{\hat{\nu}}
\newcommand{\xihat}{\hat{\xi}}
\newcommand{\pihat}{\hat{\pi}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\sighat}{\hat{\sigma}}
\newcommand{\sigmahat}{\hat{\sigma}}
\newcommand{\tauhat}{\hat{\tau}}
\newcommand{\upsilonhat}{\hat{\upsilon}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\chihat}{\hat{\chi}}
\newcommand{\psihat}{\hat{\psi}}
\newcommand{\omegahat}{\hat{\omega}}

\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\betatil}{\tilde{\beta}}
\newcommand{\gatil}{\tilde{\gamma}}
\newcommand{\gammatil}{\tilde{\gamma}}
\newcommand{\deltatil}{\tilde{\delta}}
\newcommand{\epstil}{\tilde{\epsilon}}
\newcommand{\epsilontil}{\tilde{\epsilon}}
\newcommand{\zetil}{\tilde{\zeta}}
\newcommand{\zetatil}{\tilde{\zeta}}
\newcommand{\etatil}{\tilde{\eta}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\iotatil}{\tilde{\iota}}
\newcommand{\kappatil}{\tilde{\kappa}}
\newcommand{\lambdatil}{\tilde{\lambda}}
\newcommand{\mutil}{\tilde{\mu}}
\newcommand{\nutil}{\tilde{\nu}}
\newcommand{\xitil}{\tilde{\xi}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\rhotil}{\tilde{\rho}}
\newcommand{\sigtil}{\tilde{\sigma}}
\newcommand{\sigmatil}{\tilde{\sigma}}
\newcommand{\tautil}{\tilde{\tau}}
\newcommand{\upsilontil}{\tilde{\upsilon}}
\newcommand{\phitil}{\tilde{\phi}}
\newcommand{\chitil}{\tilde{\chi}}
\newcommand{\psitil}{\tilde{\psi}}
\newcommand{\omegatil}{\tilde{\omega}}

\newcommand{\alphat}{\tilde{\alpha}}
\newcommand{\betat}{\tilde{\beta}}
\newcommand{\gammat}{\tilde{\gamma}}
\newcommand{\deltat}{\tilde{\delta}}
\newcommand{\epsilont}{\tilde{\epsilon}}
\newcommand{\epst}{\tilde{\epsilon}}
\newcommand{\zetat}{\tilde{\zeta}}
\newcommand{\etat}{\tilde{\eta}}
\newcommand{\thetat}{\tilde{\theta}}
\newcommand{\iotat}{\tilde{\iota}}
\newcommand{\kappat}{\tilde{\kappa}}
\newcommand{\lambdat}{\tilde{\lambda}}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\nut}{\tilde{\nu}}
\newcommand{\xit}{\tilde{\xi}}
\newcommand{\pit}{\tilde{\pi}}
\newcommand{\rhot}{\tilde{\rho}}
\newcommand{\sigt}{\tilde{\sigma}}
\newcommand{\sigmat}{\tilde{\sigma}}
\newcommand{\taut}{\tilde{\tau}}
\newcommand{\upsilont}{\tilde{\upsilon}}
\newcommand{\phit}{\tilde{\phi}}
\newcommand{\chit}{\tilde{\chi}}
\newcommand{\psit}{\tilde{\psi}}
\newcommand{\omegat}{\tilde{\omega}}

% Upper Case Greek Symbols
\newcommand{\Gammabar}{\bar{\Gamma}}
\newcommand{\Deltabar}{\bar{\Delta}}
\newcommand{\Thetabar}{\bar{\Theta}}
\newcommand{\Lambdabar}{\bar{\Lambda}}
\newcommand{\Xibar}{\bar{\Xi}}
\newcommand{\Pibar}{\bar{\Pi}}
\newcommand{\Sigmabar}{\bar{\Sigma}}
\newcommand{\Upsilonbar}{\bar{\Upsilon}}
\newcommand{\Phibar}{\bar{\Phi}}
\newcommand{\Psibar}{\bar{\Psi}}
\newcommand{\Omegabar}{\bar{\Omega}}

\newcommand{\Gammahat}{\hat{\Gamma}}
\newcommand{\Deltahat}{\hat{\Delta}}
\newcommand{\Thetahat}{\hat{\Theta}}
\newcommand{\Lambdahat}{\hat{\Lambda}}
\newcommand{\Xihat}{\hat{\Xi}}
\newcommand{\Pihat}{\hat{\Pi}}
\newcommand{\Sigmahat}{\hat{\Sigma}}
\newcommand{\Upsilonhat}{\hat{\Upsilon}}
\newcommand{\Phihat}{\hat{\Phi}}
\newcommand{\Psihat}{\hat{\Psi}}
\newcommand{\Omegahat}{\hat{\Omega}}

\newcommand{\Gammatil}{\tilde{\Gamma}}
\newcommand{\Deltatil}{\tilde{\Delta}}
\newcommand{\Thetatil}{\tilde{\Theta}}
\newcommand{\Lambdatil}{\tilde{\Lambda}}
\newcommand{\Xitil}{\tilde{\Xi}}
\newcommand{\Pitil}{\tilde{\Pi}}
\newcommand{\Sigmatil}{\tilde{\Sigma}}
\newcommand{\Upsilontil}{\tilde{\Upsilon}}
\newcommand{\Phitil}{\tilde{\Phi}}
\newcommand{\Psitil}{\tilde{\Psi}}
\newcommand{\Omegatil}{\tilde{\Omega}}

\newcommand{\Gammatilde}{\widetilde{\Gamma}}
\newcommand{\Deltatilde}{\widetilde{\Delta}}
\newcommand{\Thetatilde}{\widetilde{\Theta}}
\newcommand{\Lambdatilde}{\widetilde{\Lambda}}
\newcommand{\Xitilde}{\widetilde{\Xi}}
\newcommand{\Pitilde}{\widetilde{\Pi}}
\newcommand{\Sigmatilde}{\widetilde{\Sigma}}
\newcommand{\Upsilontilde}{\widetilde{\Upsilon}}
\newcommand{\Phitilde}{\widetilde{\Phi}}
\newcommand{\Psitilde}{\widetilde{\Psi}}
\newcommand{\Omegatilde}{\widetilde{\Omega}}

\newcommand{\Gammat}{\tilde{\Gamma}}
\newcommand{\Deltat}{\tilde{\Delta}}
\newcommand{\Thetat}{\tilde{\Theta}}
\newcommand{\Lambdat}{\tilde{\Lambda}}
\newcommand{\Xit}{\tilde{\Xi}}
\newcommand{\Pit}{\tilde{\Pi}}
\newcommand{\Sigmat}{\tilde{\Sigma}}
\newcommand{\Upsilont}{\tilde{\Upsilon}}
\newcommand{\Phit}{\tilde{\Phi}}
\newcommand{\Psit}{\tilde{\Psi}}
\newcommand{\Omegat}{\tilde{\Omega}}

% others
\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\delbar}{\bar{\delta}}

\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}


%%%% Symbols specific to this project %%%%%

\newcommand{\Poisson}{\mathrm{Poisson}}

